TLIO: Tight Learned Inertial Odometry

In this work we propose a tightly-coupled Extended Kalman Filter framework for IMU-only state estimation. Strap-down IMU measurements provide relative state estimates based on IMU kinematic motion model. However the integration of measurements is sensitive to sensor bias and noise, causing significant drift within seconds. Recent research by Yan et al. (RoNIN) and Chen et al. (IONet) showed the capability of using trained neural networks to obtain accurate 2D displacement estimates from segments of IMU data and obtained good position estimates from concatenating them. This paper demonstrates a network that regresses 3D displacement estimates and its uncertainty, giving us the ability to tightly fuse the relative state measurement into a stochastic cloning EKF to solve for pose, velocity and sensor biases. We show that our network, trained with pedestrian data from a headset, can produce statistically consistent measurement and uncertainty to be used as the update step in the filter, and the tightly-coupled system outperforms velocity integration approaches in position estimates, and AHRS attitude filter in orientation estimates.

==> macros/macro_alphabet.tex <==
% Document LaTeX	Auteur : Guy Le Besnerais	Date : 25/05/94
% Modification : J.-F. Gio	(15/09/95)
%			        J.I. (format Latex 2e, taille adaptative 22/03/99)
%			             (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}

\def\sbm#1{\ensuremath{\boldsymbol{#1}}}         % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}             % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}             % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}         % Style cursif
\def\scb#1{\ensuremath{\mathbf{\mathcal{#1}}}}   % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}            % Style blackboard (necessite bbm)

%---- NEW - NEW ---- Small caps gras ---- 05-06-98 ---- JFG ------
%----------------- Merci \`a Caro --------------------------------
\DeclareFontShape{T1}{cmr}{bx}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}
% SC en bold (Hack !)
\DeclareFontShape{T1}{cmr}{b}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}%
\def\scb#1{\bfseries {\scshape #1}}%

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS
\XS

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  %\def\sb{{\sbm{s}}\XS} this breaks prescript
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}	\def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}	\def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}	\def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}	\def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}	\def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}	\def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}	\def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}	\def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}	\def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}	\def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}	\def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}	\def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}	\def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}	\def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}	\def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}	\def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}	\def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}	\def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}	\def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}	\def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}	\def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}	\def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}	\def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}	\def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}	\def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}	\def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS, taille adaptative

\def\alphab      {{\sbm{\alpha}}\XS}
\def\betab       {{\sbm{\beta}}\XS}
\def\gammab      {{\sbm{\gamma}}\XS}	  \def\Gammab    {{\sbm{\Gamma}}\XS}
\def\deltab      {{\sbm{\delta}}\XS}	  \def\Deltab    {{\sbm{\Delta}}\XS}
\def\epsilonb    {{\sbm{\epsilon}}\XS}
\def\varepsilonb {{\sbm{\varepsilon}}\XS}
\def\etab        {{\sbm{\eta}}\XS}
\def\thetab      {{\sbm{\theta}}\XS}	  \def\Thetab    {{\sbm{\Theta}}\XS}
\def\varthetab   {{\sbm{\vartheta}}\XS}
\def\iotab       {{\sbm{\iota}}\XS}
\def\kappab      {{\sbm{\kappa}}\XS}
\def\lambdab     {{\sbm{\lambda}}\XS}    \def\Lambdab   {{\sbm{\Lambda}}\XS}
\def\mub         {{\sbm{\mu}}\XS}
\def\nub         {{\sbm{\nu}}\XS}
\def\xib         {{\sbm{\xi}}\XS}		  \def\Xib  	  {{\sbm{\Xi}}\XS}
\def\pib         {{\sbm{\pi}}\XS}		  \def\Pib  	  {{\sbm{\Pi}}\XS}
\def\varpib      {{\sbm{\varpi}}\XS}
\def\rhob        {{\sbm{\rho}}\XS}
\def\varrhob     {{\sbm{\varrho}}\XS}
\def\sigmab      {{\sbm{\sigma}}\XS}	  \def\Sigmab    {{\sbm{\Sigma}}\XS}
\def\varsigmab   {{\sbm{\varsigma}}\XS}  \def\Varsigmab {{\sbm{\Varsigma}}\XS}
\def\phib        {{\sbm{\phi}}\XS}  	  \def\Phib 	  {{\sbm{\Phi}}\XS}
\def\varphib     {{\sbm{\varphi}}\XS}
\def\chib        {{\sbm{\chi}}\XS}
\def\psib        {{\sbm{\psi}}\XS}  	  \def\Psib 	  {{\sbm{\Psi}}\XS}
\def\omegab      {{\sbm{\omega}}\XS}	  \def\Omegab    {{\sbm{\Omega}}\XS}
\def\taub        {{\sbm{\tau}}\XS}
\def\upsilonb    {{\sbm{\upsilon}}\XS}   \def\Upsilonb  {{\sbm{\Upsilon}}\XS}
\def\zetab       {{\sbm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{0}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}


